Desiderata for Representation Learning: A Causal Perspective

Representation learning constructs low-dimensional representations to summarize essential features of high-dimensional data. This learning problem is often approached by describing various desiderata associated with learned representations; e.g., that they be non-spurious, efficient, or disentangled. It can be challenging, however, to turn these intuitive desiderata into formal criteria that can be measured and enhanced based on observed data. In this paper, we take a causal perspective on representation learning, formalizing non-spuriousness and efficiency (in supervised representation learning) and disentanglement (in unsupervised representation learning) using counterfactual quantities and observable consequences of causal assertions. This yields computable metrics that can be used to assess the degree to which representations satisfy the desiderata of interest and learn non-spurious and disentangled representations from single observational datasets.

==> img/causal-representation-scm-id-orig.tex <==
% !TEX root = ../representation-causal.tex
\begin{tikzpicture}
% \tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1, dashed]
[obs/.style={draw,circle,filled,minimum size=1cm}, latent/.style={draw,circle,minimum size=1cm}]
  % Define nodes
  \node[latent] (u) {$\mbC$};
  % \node[obs, below=1.2cm of u, xshift=2cm] (gd) {$G_d$};
  % \node[obs, below=1.2cm of u, xshift=-2cm] (g1) {$G_1$};
  %   \node[obs, below=1.2cm of u, xshift=-0cm] (g2) {$G_2$};
  \node[obs, below=1.2cm of u, xshift=3cm] (am) {$X_m$};
  \node[obs, below=1.2cm of u, xshift=-4cm] (a1) {$X_1$};
  \node[obs, below=1.2cm of u, xshift=-2cm] (a2) {$X_2$};
  % \node[latent, below=3.5cm of u, xshift=0cm] (z) {$\mbZ$};
  \node[obs, below=3.5cm of u, xshift=0cm] (y) {$Y$};
  % Connect the nodes
  \edge{u}{a1,a2,am};
  \edge{am}{y};
  \edge{a1}{y};
  \edge{a2}{y};
  % \edge{z}{y};
  % \edge{g1}{a1,a2,am};
  % \edge{g2}{a1,a2,am};
  % \edge{gd}{a1,a2,am};
  % \node at ($(g2)!.5!(gd)$) {\ldots};
  \node at ($(a2)!.5!(am)$) {\ldots \quad \ldots};
\end{tikzpicture}


==> img/causal-representation-scm-id.tex <==
% !TEX root = ../representation-causal.tex
\begin{tikzpicture}
% \tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1, dashed]
[obs/.style={draw,circle,filled,minimum size=1cm}, latent/.style={draw,circle,minimum size=1cm}]
  % Define nodes
  \node[latent] (u) {$\mbC$};
  % \node[obs, below=1.2cm of u, xshift=2cm] (gd) {$G_d$};
  % \node[obs, below=1.2cm of u, xshift=-2cm] (g1) {$G_1$};
  %   \node[obs, below=1.2cm of u, xshift=-0cm] (g2) {$G_2$};
  \node[obs, below=1.2cm of u, xshift=3cm] (am) {$X_m$};
  \node[obs, below=1.2cm of u, xshift=-4cm] (a1) {$X_1$};
  \node[obs, below=1.2cm of u, xshift=-2cm] (a2) {$X_2$};
  \node[latent, xshift=3cm] (z) {$\mbZ$};
  \node[obs, below=3.5cm of u, xshift=0cm] (y) {$Y$};
  % Connect the nodes
  \edge{u}{a1,a2,am, z};
  \edge{am}{y};
  \edge{a1}{y};
  \edge{a2}{y};
  \edge{z}{a1, a2, am};
  % \edge{g1}{a1,a2,am};
  % \edge{g2}{a1,a2,am};
  % \edge{gd}{a1,a2,am};
  % \node at ($(g2)!.5!(gd)$) {\ldots};
  \node at ($(a2)!.5!(am)$) {\ldots \quad \ldots};
\end{tikzpicture}


==> img/causal-representation-scm.tex <==
% !TEX root = ../representation-causal.tex
\begin{tikzpicture}
% \tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1, dashed]
[obs/.style={draw,circle,filled,minimum size=1cm}, latent/.style={draw,circle,minimum size=1cm}]
  % Define nodes
  \node[latent] (u) {$\mbC$};
  \node[latent, below=1.2cm of u, xshift=2cm] (gd) {$Z_d$};
  \node[latent, below=1.2cm of u, xshift=-2cm] (g1) {$Z_1$};
    \node[latent, below=1.2cm of u, xshift=-0cm] (g2) {$Z_2$};
  \node[obs, below=1.2cm of g2, xshift=3cm] (am) {$X_m$};
  \node[obs, below=1.2cm of g2, xshift=-4cm] (a1) {$X_1$};
  \node[obs, below=1.2cm of g2, xshift=-2cm] (a2) {$X_2$};
  % \node[latent, below=3.5cm of u, xshift=0cm] (z) {$\mbZ$};
  \node[obs, below=1.2cm of a2, xshift=2cm] (y) {$Y$};
  % Connect the nodes
  \edge{u}{g1,g2,gd};
  \edge{am}{y};
  \edge{a1}{y};
  \edge{a2}{y};
  % \edge{z}{y};
  \edge{g1}{a1,a2,am};
  \edge{g2}{a1,a2,am};
  \edge{gd}{a1,a2,am};
  \node at ($(g2)!.5!(gd)$) {\ldots};
  \node at ($(a2)!.5!(am)$) {\ldots \quad \ldots};
\end{tikzpicture}


==> img/disentangle-scm.tex <==
% !TEX root = ../disentangle-notes.tex
\begin{tikzpicture}
% \tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1, dashed]
[obs/.style={draw,circle,filled,minimum size=1cm}, latent/.style={draw,circle,minimum size=1cm}]
  % Define nodes
  \node[latent] (u) {$\mbC$};
  \node[latent, below=1.2cm of u, xshift=2cm] (gd) {$Z_d$};
  \node[latent, below=1.2cm of u, xshift=-2cm] (g1) {$Z_1$};
    \node[latent, below=1.2cm of u, xshift=-0cm] (g2) {$Z_2$};
  \node[obs, below=3.5cm of u, xshift=3cm] (am) {$X_m$};
  \node[obs, below=3.5cm of u, xshift=-4cm] (a1) {$X_1$};
  \node[obs, below=3.5cm of u, xshift=-2cm] (a2) {$X_2$};
  % Connect the nodes
  \edge{u}{g1,g2,gd};
  \edge{g1}{a1,a2,am};
  \edge{g2}{a1,a2,am};
  \edge{gd}{a1,a2,am};
  \node at ($(g2)!.5!(gd)$) {\ldots};
  \node at ($(a2)!.5!(am)$) {\ldots \quad \ldots};
\end{tikzpicture}


==> synthetic-text-words.tex <==
% !TEX root = causal_rep.tex


\begin{table}[t]
    \centering
    \begin{tabular}{lp{0.4\linewidth}  p{0.4\linewidth}}
      &CAUSAL-REP  & Linear Regression \\ \hline
      1& great\_use; worth\_penny; excellent\_product; wont\_disappointed; glad\_bought; referral; best\_phone; great\_product; pleased; activated; works\_great; great\_camera;
      & wont\_disappointed; great\_product; amazing; referral; software; excellent; works\_advertised; easy; dont; awsome; awesome; penny; \\
      2 & waste; waste\_money; worst; junk; stay\_away; disappointing; refund; returning; useless; repair; poor\_quality;  
      &  pretty; overall; waste; stars; junk; needless\_say; lcd; awful; stopped; probably; description; volume; \\
    \end{tabular}
    \caption{CAUSAL-REP learns representation that relies less on words
    spuriously correlated with the sentiment. The table shows the top
    12 words identified by the two-dimensional representation. The
    representation obtained from the naive algorithm involves more
    words that are spuriously correlated with the sentiment; e.g.,
    ``software,'' ``penny,'' ``needless\_say,'' and ``lcd.''}
    \label{tab:amazon-reviews}
\end{table}



==> table_causalrep_sim.tex <==
% !TEX root = causal_rep.tex

\begin{table*}[t]
\scriptsize
\begin{center}
\begin{tabular}{lp{9mm}p{9mm}p{9mm}p{9mm}p{9mm}p{15mm}} 
\toprule
ID $(i)$ & px\_1 $(x_{i1})$ & px\_2 $(x_{i2})$& px\_3 $(x_{i3})$&  px\_4 $(x_{i4})$& px\_5 $(x_{i5})$ & brightness $(y_i)$\\
\midrule
1 & 1 & 0 & 0 & 1 & & 5.73\\
2 & 1 & 2 & 2 & 1 & & 5.26\\
3 & 2 & 0 & 1 & 1 & & 6.24\\
4 & 0 & 0 & 0 & 1 & & 5.78\\
5 & 1 & 2 & 1 & 1 & & 5.09 \\
$\vdots$ &  & & $\vdots$&  & & $\vdots$ \\
\bottomrule
\end{tabular}
\caption{Learning representations of pixel values for brightness labels.\label{tab:tab_causalrep_sim}}
\end{center}
\end{table*}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

